ZeroFlow: Scalable Scene Flow via Distillation

Scene flow estimation is the task of describing the 3D motion field between temporally successive point clouds. State-of-the-art methods use strong priors and test-time optimization techniques, but require on the order of tens of seconds to process full-size point clouds, making them unusable as computer vision primitives for real-time applications such as open world object detection. Feedforward methods are considerably faster, running on the order of tens to hundreds of milliseconds for full-size point clouds, but require expensive human supervision. To address both limitations, we propose Scene Flow via Distillation, a simple, scalable distillation framework that uses a label-free optimization method to produce pseudo-labels to supervise a feedforward model. Our instantiation of this framework, ZeroFlow, achieves state-of-the-art performance on the Argoverse 2 Self-Supervised Scene Flow Challenge while using zero human labels by simply training on large-scale, diverse unlabeled data. At test-time, ZeroFlow is over 1000x faster than label-free state-of-the-art optimization-based methods on full-size point clouds (34 FPS vs 0.028 FPS) and over 1000x cheaper to train on unlabeled data compared to the cost of human annotation (\$394 vs ~\$750,000). To facilitate further research, we release our code, trained model weights, and high quality pseudo-labels for the Argoverse 2 and Waymo Open datasets at https://vedder.io/zeroflow.html

==> tikz_figures/scene_flow_example.tex <==
\begin{tikzpicture}
    \setlength{\fboxsep}{0.0pt}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\fbox{\includegraphics[width=0.47\textwidth]{screenshot_figures/qualitative/argo/white_bg/gt_flow_cropped.png}}};
    \node[anchor=south west,inner sep=0] (image2) at (6.9,0) {\fbox{\includegraphics[width=0.47\textwidth]{screenshot_figures/qualitative/argo/white_bg/our_flow_cropped.png}}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
      % Define the zoom area
      \coordinate (zoom_area_south_west) at (0.52,0.63);
      \coordinate (zoom_area_north_east) at (0.66,0.75);
      \coordinate (zoom_area_north_west) at (0.52,0.75);

      % Draw the zoom area rectangle
      \draw[black] (zoom_area_south_west) rectangle (zoom_area_north_east);

      % Draw the zoomed image
      \node[inner sep=0,right=-1.6cm of image, yshift=0.8cm] (zoomed_image) {{\fbox{\includegraphics[width=3.2cm]{screenshot_figures/qualitative/argo/white_bg/close_up_cropped_small.png}}}};

      % Draw the zoom lines
      \draw[black] (zoom_area_south_west) -- (zoomed_image.south west);
      \draw[black] (zoom_area_north_west) -- (zoomed_image.north west);
    \end{scope}
  \end{tikzpicture}
